The Second Monocular Depth Estimation Challenge

This paper discusses the results for the second edition of the Monocular Depth Estimation Challenge (MDEC). This edition was open to methods using any form of supervision, including fully-supervised, self-supervised, multi-task or proxy depth. The challenge was based around the SYNS-Patches dataset, which features a wide diversity of environments with high-quality dense ground-truth. This includes complex natural environments, e.g. forests or fields, which are greatly underrepresented in current benchmarks. The challenge received eight unique submissions that outperformed the provided SotA baseline on any of the pointcloud- or image-based metrics. The top supervised submission improved relative F-Score by 27.62%, while the top self-supervised improved it by 16.61%. Supervised submissions generally leveraged large collections of datasets to improve data diversity. Self-supervised submissions instead updated the network architecture and pretrained backbones. These results represent a significant progress in the field, while highlighting avenues for future research, such as reducing interpolation artifacts at depth boundaries, improving self-supervised indoor performance and overall natural image accuracy.

==> Figures/depth.tex <==
% SYNS-Patches Depth Visualizations

\tiny

\def\first{0143}
\def\nums{0535,0296,0372,0195,0247,0731,0761}
\def\dataset{SynsDepth}

\def\second{0556}
\def\numss{0226,0044,0051,0656,0462,0739,0747}
\def\datasett{SynsDepth2}


\def\methods{
    img/
    ,gt/GT
    ,jspenmar/\team{0}
    ,KaiCheng/\team{1}
    ,xiangmochu/\team{2}
    ,ch977/\team{3}
    ,tkl/\team{5}
    ,LBJ/\team{6}
    ,myungwoo/\team{4}
    ,cqzhao/\team{7}
    ,Tutu_inv/\team{8}
}

\def\w{0.12\linewidth}

\foreach \method/\label in \methods{%
    \begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0,anchor=south west}]
        \node (image) at (0, 0) {\includegraphics[width=\w]{\dataset/\first_\method.jpeg}};
        \begin{scope}[x={(image.south east)},y={(image.north west)}]
            \draw (0.01, 0.01) node {\color{white}{\textbf{\label}}};
        \end{scope}
    \end{tikzpicture}
    %
    \foreach \num in \nums{%
        \includegraphics[width=\w]{\dataset/\num_\method.jpeg}
    } \\
}

\vspace{1em}

\foreach \method/\label in \methods{%
    \begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0,anchor=south west}]
        \node (image) at (0, 0) {\includegraphics[width=\w]{\datasett/\second_\method.jpeg}};
        \begin{scope}[x={(image.south east)},y={(image.north west)}]
            \draw (0.01, 0.01) node {\color{white}{\textbf{\label}}};
        \end{scope}
    \end{tikzpicture}
    %
    \foreach \num in \numss{%
        \includegraphics[width=\w]{\datasett/\num_\method.jpeg}
    } \\
}

\mycaption{\acl{syns} Depth Visualization}{%
Best viewed in color and zoomed in.
Most methods struggle with thin structures, such as branches and railings. 
Object boundaries are also characterized by ``halos'', caused by interpolation between foreground and background objects. 
Notable improvements can be seen in Natural and Agricultural scenes, where the top submissions provide much higher levels of detail than the baseline. 
}


==> Figures/distrib.tex <==
% SYNS-Patches Depth Distribution

\includegraphics[width=1\linewidth]{Images/depth_distrib.pdf}

\mycaption{Depth Distribution Per Scene Type}{%
Indoor scenes are limited to 20m, while outdoor scenes reach up to 120m. 
Natural and Agriculture scenes contain a larger percentage of long-range depths (20-80m), while urban scenes focus on the mid-range (20-40m).
}


==> Figures/syns.tex <==
% SYNS-Patches Sample Images

\foreach \img in {img, gt, edge}{%
    \foreach \num in {0064, 0131, 0156, 0183}{%
        \includegraphics[width=0.25\linewidth]{Syns/\num_\img.jpeg}%
    }\\\vspace{-1pt}%
}
\vspace{0.1cm}
\foreach \img in {img, gt, edge}{%
    \foreach \num in {0234, 0337, 0352, 0367}{%
        \includegraphics[width=0.25\linewidth]{Syns/\num_\img.jpeg}%
    }\\\vspace{-1pt}%
}

\mycaption{\acl{syns}}{%
Sample images from the diverse dataset scenes, including complex urban, natural and indoor settings. 
The dataset contains high-quality ground-truth with 78.20\% coverage. 
Depth boundaries were computed as Canny edges in the log-depth maps. 
}


==> Tables/datasets.tex <==
% Dataset Statistics

\mycaption{Dataset \& Benchmark Comparison}{%
We summarize recent datasets commonly used in self-supervised monocular depth estimation. 
CityScapes represents a common pretraining dataset, while \acl{syns} is testing-only.
\acl{syns} is the only dataset providing high-quality dense depth maps in a wide variety of environments.
}

\begin{tabular}{llllllllll}
\toprule
                                                  &    Accuracy & Density (\%) &  Num Points &  Urban & Natural &  Indoor &   Train &     Val &    Test \\
\midrule
                     CityScapes~\cite{Cordts2016} &      \xmark &       \xmark &      \xmark & \cmark &  \xmark &  \xmark &  88,250 &  \xmark &  \xmark \\
      Kitti Eigen-Zhou~\cite{Geiger2013,Zhou2017} &      \xmark &       \xmark &      \xmark & \cmark &  \xmark &  \xmark &  39,810 &   4,424 &  \xmark \\
\midrule
          Kitti Eigen~\cite{Geiger2013,Eigen2015} &         Mid &         4.10 &         19k & \cmark &  \xmark &  \xmark &  45,200 &   1,776 &     697 \\
Kitti Eigen-Benchmark~\cite{Geiger2013,Uhrig2018} &        High &        15.28 &         71k & \cmark &  \xmark &  \xmark &  71,633 &   5,915 &     652 \\
                        DDAD~\cite{Guizilini2020} &        High &         1.02 &         24k & \cmark &  \xmark &  \xmark &  75,900 &  23,700 &   3,080 \\
\midrule
          \acl{syns}~\cite{Adams2016,Spencer2022} &        High &        78.30 &        365k & \cmark &  \cmark &  \cmark &  \xmark &     400 &     775 \\
\bottomrule
\end{tabular}


==> Tables/results.tex <==
% SYNS-Patches Results

\footnotesize

\def\n{9}

\mycaption{\acl{syns} Results}{%
We provide metrics across the whole dataset and per scene-category. 
As expected, supervised methods generally outperform self-supervised ones. 
The largest gap can be found in Indoor scenes, self-supervised methods were trained exclusively on automotive data. 
Teams~\team{4} \& \team{5} outperformed the challenge baseline~\cite{Spencer2022} by incorporating more advanced network architectures.
}

\begin{tabular}{@{}lllllllllll@{}}
\toprule
                                           &            & Train & Rank &        F\up & F-Edges\up &     MAE\down &    RMSE\down &      AbsRel\down & Acc-Edges\down & Comp-Edges\down \\ 
\midrule           
            
            \multirow{\n}*{\emph{Overall}} &  \team{1} & \train{1} &  \best{1} &  \best{17.51} &         8.80 &  \best{4.52} &         8.72 &  \best{24.32} &         3.22 &         21.65 \\ 
                                           &  \team{2} & \train{3} & \nbest{2} & \nbest{16.94} &  \best{9.63} & \nbest{4.71} &  \best{8.00} &         25.35 &         3.56 &         19.95 \\ 
                                           &  \team{3} & \train{3} &         3 &         16.70 & \nbest{9.36} &         4.91 &         8.63 & \nbest{24.33} &  \best{3.02} &         18.07 \\ 
                                           &  \team{5} & \train{5} &         4 &         16.00 &         8.49 &         5.08 &         8.96 &         28.46 &         3.74 &  \best{11.32} \\ 
                                           &  \team{6} & \train{6} &         5 &         14.71 &         8.13 &         5.17 &         8.97 &         29.43 &         3.75 & \nbest{17.29} \\ 
                                           &  \team{0} & \train{0} &         6 &         13.72 &         7.76 &         5.56 &         9.72 &         32.04 &         3.97 &         21.63 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         13.23 &         8.26 &         5.18 &         8.76 &         28.03 & \nbest{3.07} &         29.96 \\ 
                                           &  \team{4} & \train{4} &         7 &         12.77 &         7.68 &         5.17 &         8.83 &         29.92 &         3.56 &         35.26 \\ 
                                           &  \team{7} & \train{7} &         8 &         12.44 &         7.49 &         5.05 & \nbest{8.59} &         28.99 & \nbest{3.10} &         38.93 \\ 
                                           &  \team{8} & \train{8} &        9 &         11.29 &         7.18 &         5.81 &         9.58 &         32.82 &         3.47 &         43.38 \\ 
                                        %   &\team{10} & \train{10} &        11 &          9.99 &         6.74 &         5.95 &         9.69 &         34.49 &         3.51 &         47.95 \\ 
\midrule
      \multirow{\n}*{\emph{Outdoor-Urban}} &  \team{1} & \train{1} &  \best{1} &  \best{16.41} &         7.37 &  \best{3.81} &         7.82 &  \best{21.85} &         2.91 &         24.36 \\ 
                                           &  \team{5} & \train{5} &         4 & \nbest{16.28} &         7.27 &         4.49 &         7.98 &         26.18 &         3.67 &  \best{13.11} \\ 
                                           &  \team{6} & \train{6} &         5 &         15.21 &         6.80 &         4.60 &         8.00 &         27.55 &         3.73 &         16.26 \\ 
                                           &  \team{2} & \train{3} & \nbest{2} &         15.10 &  \best{8.48} & \nbest{4.03} &  \best{6.90} &         23.67 &         3.36 &         19.13 \\ 
                                           &  \team{3} & \train{3} &         3 &         15.01 & \nbest{7.79} &         4.26 &         7.70 & \nbest{22.88} & \nbest{2.87} & \nbest{15.73} \\ 
                                           &  \team{0} & \train{0} &         6 &         14.09 &         6.48 &         4.77 &         8.43 &         29.10 &         3.89 &         22.75 \\ 
                                           &  \team{4} & \train{4} &         7 &         12.90 &         5.92 &         4.49 &         7.80 &         27.44 &         3.26 &         35.36 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         12.53 &         6.43 &         4.61 &         7.93 &         26.28 &  \best{2.82} &         27.07 \\ 
                                           &  \team{7} & \train{7} &         8 &         12.52 &         5.89 &         4.37 & \nbest{7.62} &         26.46 &  \best{2.83} &         40.33 \\ 
                                           &  \team{8} & \train{8} &         9 &         11.31 &         5.73 &         5.14 &         8.69 &         30.64 &         3.13 &         40.15 \\ 
                                        %   &\team{10} & \train{10} &        11 &          9.95 &         5.18 &         5.20 &         8.73 &         32.12 &         3.15 &         43.54 \\ 
\midrule   
    \multirow{\n}*{\emph{Outdoor-Natural}} &  \team{2} & \train{3} & \nbest{2} &  \best{14.90} & \nbest{6.75} & \nbest{6.26} &  \best{10.47} &         28.40 &         3.54 &         14.44 \\ 
                                           &  \team{3} & \train{3} &         3 & \nbest{14.66} &  \best{6.79} &         6.35 &         10.86 & \nbest{27.09} &  \best{3.08} &         19.73 \\ 
                                           &  \team{5} & \train{5} &         4 &         14.43 &         6.02 &         6.51 &         11.43 &         30.57 &         3.59 &   \best{9.44} \\ 
                                           &  \team{1} & \train{1} &  \best{1} &         14.31 &         6.07 &  \best{5.97} & \nbest{10.81} &  \best{26.48} &         3.45 &         17.75 \\ 
                                           &  \team{6} & \train{6} &         5 &         12.89 &         5.74 &         6.77 &         11.62 &         32.57 &         3.68 & \nbest{13.97} \\ 
                                           &  \team{0} & \train{0} &         6 &         12.10 &         5.32 &         7.46 &         12.86 &         36.89 &         3.84 &         18.35 \\ 
                                           &  \team{4} & \train{4} &         7 &         11.54 &         6.03 &         6.87 &         11.52 &         33.66 &         3.36 &         32.47 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         11.28 &         6.12 &         6.75 &         11.02 &         32.03 & \nbest{3.09} &         28.65 \\ 
                                           &  \team{7} & \train{7} &         8 &         10.98 &         5.38 &         6.66 &         11.13 &         32.19 & \nbest{3.13} &         36.01 \\ 
                                           &  \team{8} & \train{8} &         9 &          9.26 &         4.92 &         7.69 &         12.22 &         38.14 &         3.36 &         42.92 \\ 
                                        %   &\team{10} & \train{10} &        11 &          7.73 &         4.33 &         7.91 &         12.41 &         40.51 &         3.39 &         47.33 \\ 
\midrule   
\multirow{\n}*{\emph{Outdoor-Agriculture}} &  \team{1} & \train{1} &  \best{1} &  \best{16.36} &         5.24 &  \best{5.17} &        10.13 &         29.07 &         3.43 &         18.84 \\ 
                                           &  \team{2} & \train{3} & \nbest{2} & \nbest{15.58} &  \best{6.40} & \nbest{5.25} &  \best{9.09} & \nbest{27.45} &         3.64 &         18.30 \\ 
                                           &  \team{5} & \train{5} &         4 &         14.94 &         5.49 &         5.70 &        10.14 &         30.70 &         3.75 &  \best{10.27} \\ 
                                           &  \team{3} & \train{3} &         3 &         14.68 & \nbest{5.82} &         5.61 &        10.02 &  \best{25.90} &  \best{3.17} &         17.67 \\ 
                                           &  \team{6} & \train{6} &         5 &         14.03 &         5.06 &         5.65 &         9.98 &         30.40 &         3.80 & \nbest{15.94} \\ 
                                        %   &  \team{9} & \train{9} &         7 &         12.67 &         4.92 &         5.76 &        10.04 &         29.48 &         3.18 &         29.39 \\ 
                                           &  \team{0} & \train{0} &         6 &         12.26 &         4.76 &         6.10 &        10.84 &         33.58 &         4.00 &         18.73 \\ 
                                           &  \team{4} & \train{4} &         7 &         11.56 &         4.55 &         5.61 &         9.79 &         31.16 &         3.60 &         35.30 \\ 
                                           &  \team{7} & \train{7} &         8 &         11.15 &         4.52 &         5.62 & \nbest{9.61} &         31.43 & \nbest{3.17} &         39.06 \\ 
                                           &  \team{8} & \train{8} &         9 &         10.27 &         3.97 &         6.34 &        10.76 &         33.61 &         3.40 &         38.73 \\ 
                                        %   &\team{10} & \train{10} &        11 &          8.42 &         3.41 &         6.52 &        10.91 &         35.61 &         3.42 &         43.22 \\ 
\midrule   
            \multirow{\n}*{\emph{Indoor}}  &  \team{1} & \train{1} &  \best{1} &  \best{33.20} & \nbest{33.12} &  \best{0.70} &         1.63 &  \best{13.08} &  \best{2.89} &         33.52 \\ 
                                           &  \team{3} & \train{3} &         3 & \nbest{33.08} &  \best{33.57} &         0.87 & \nbest{1.35} &         16.52 & \nbest{2.90} & \nbest{21.76} \\ 
                                           &  \team{2} & \train{3} & \nbest{2} &         32.05 &         32.53 & \nbest{0.83} &  \best{1.26} & \nbest{16.00} &         4.11 &         45.68 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         22.55 &         31.29 &         0.85 & \nbest{1.27} &         17.90 &         3.49 &         45.80 \\ 
                                           &  \team{5} & \train{5} &         4 &         22.49 &         29.53 &         1.06 &         1.59 &         23.38 &         4.38 &  \best{14.52} \\ 
                                           &  \team{0} & \train{0} &         6 &         21.11 &         28.96 &         1.04 &         1.51 &         22.77 &         4.60 &         37.09 \\ 
                                        %   & \team{10} & \train{10} &        11 &         20.84 &         29.76 &         1.03 &         1.49 &         21.12 &         5.40 &         78.85 \\ 
                                           &  \team{6} & \train{6} &         5 &         20.25 &         29.52 &         1.03 &         1.48 &         23.37 &         3.96 &         35.68 \\ 
                                           &  \team{7} & \train{7} &         8 &         19.82 &         28.62 &         0.97 &         1.42 &         20.91 &         3.63 &         43.46 \\ 
                                           &  \team{8} & \train{8} &         9 &         19.81 &         28.93 &         1.02 &         1.49 &         21.83 &         5.19 &         69.50 \\ 
                                           &  \team{4} & \train{4} &         7 &         19.18 &         28.34 &         1.09 &         1.61 &         23.24 &         5.14 &         44.02 \\ 
\bottomrule
\end{tabular}

\emph{
\textbf{M}=Monocular -- \textbf{S}=Stereo -- \textbf{D*}=Proxy Depth -- \textbf{D}=Ground-truth Depth
}


==> Tables/syns_cat.tex <==

% SYNS-Patches Category Distribution

\mycaption{\acl{syns}}{Distribution of images per category in the val/test splits.}

\begin{tabular}{@{}llllllllll|l@{}}
\toprule
               & Agriculture & Indoor & Industry & Misc & Natural & Recreation & Residential & Transport & Woodland & Total \\ 
\midrule
  \textbf{Val} &         104 &     67 &       36 &   72 &      36 &         14 &          13 &         4 &       54 &   400 \\ 

 \textbf{Test} &         211 &     81 &       71 &    0 &     147 &         48 &         110 &        17 &       90 &   775 \\ 
\midrule
\textbf{Total} &         315 &    148 &      107 &   72 &     183 &         62 &         123 &        21 &      144 & 1,175 \\ 
\bottomrule
\end{tabular}

